Economic Networks: Theory and Computation

This textbook is an introduction to economic networks, intended for students and researchers in the fields of economics and applied mathematics. The textbook emphasizes quantitative modeling, with the main underlying tools being graph theory, linear algebra, fixed point theory and programming. The text is suitable for a one-semester course, taught either to advanced undergraduate students who are comfortable with linear algebra or to beginning graduate students.

==> backmatter.tex <==

%% index

%\citeindexfalse
%\printindex

%% author index

%\renewcommand{\indexname}{Author Index}
%\chapter*{Author Index}
%\begin{multicols}{3}
%\printauthorindex
%\end{multicols}




==> tikz/data_description_after_modified.tex <==
The data for the figure was obtained from the International Settlement Bank's Consolidated banking statistics, for the years 2019 Quarter 4. We used the immediate counterparty basis for financial claims of domestic and foreign banks, which calculates the sum of cross-border claims and local claims of foreign affiliates in both foreign and local currency. The foreign claim of a node to itself is set to 0. The size of each node in the figure is increasing in the total foreign claims of all other nodes on this node. The widths of the arrows are proportional to the foreign claims they represent, respectively. Additionally, all arrows representing foreign claims over US\$10 million are wiped out in the network visualization but not in centrality plots.

==> tikz/markov_switching_process.tex <==
\begin{tikzpicture}
  \node[circle, draw] (0) at (0, 0) {0};
  \node[circle, draw] (1) at (3, 0) {1};
  \draw[->, thick, black]
  (0) edge [bend left=20, above] node {$1-p$} (1)
  (1) edge [bend left=20, below] node {$1-q$} (0)
  (1) edge [loop below] node {$q$} (1)
  (0) edge [loop above] node {$p$} (0);
\end{tikzpicture}
